PolMERLIN: Self-Supervised Polarimetric Complex SAR Image Despeckling with Masked Networks

Despeckling is a crucial noise reduction task in improving the quality of synthetic aperture radar (SAR) images. Directly obtaining noise-free SAR images is a challenging task that has hindered the development of accurate despeckling algorithms. The advent of deep learning has facilitated the study of denoising models that learn from only noisy SAR images. However, existing methods deal solely with single-polarization images and cannot handle the multi-polarization images captured by modern satellites. In this work, we present an extension of the existing model for generating single-polarization SAR images to handle multi-polarization SAR images. Specifically, we propose a novel self-supervised despeckling approach called channel masking, which exploits the relationship between polarizations. Additionally, we utilize a spatial masking method that addresses pixel-to-pixel correlations to further enhance the performance of our approach. By effectively incorporating multiple polarization information, our method surpasses current state-of-the-art methods in quantitative evaluation in both synthetic and real-world scenarios.

==> sec/rebuttal.tex <==
\section{Authors response to reviewers comments}
\label{sec:response}
First, we would like to acknowledge the two reviewers and the editor for their careful and fruitful peer review.

\subsection{Reviewer 1}

\begin{quote}
This strategy seems intuitive and lacks significant novel technological advancement(s).
\end{quote}

Our main idea -- extending the existing self-supervised despeckling strategy to multiple polarization images -- might appear relatively intuitive. However, when attempting to directly apply this ``intuitive'' approach to multiple polarization images, there are multiple choices concerning the combinations of polarization images and their real and imaginary parts. Among these, which is the most optimal combination? This is a non-trivial issue that arises only when dealing with multiple complex polarization images. To address it, one must answer a question: what underlying assumptions are we making, physically, when solving this type of prediction problem? And are these assumptions valid? Unless answering this, even if the proposed method seems simple, we can only rely on empirical exploration testing to determine under what conditions it can be used, and whether it can also be applied to other multi-polarization image sensors. As described in Section 3, instead of relying on such empirical methodologies, we made clear the assumptions behind the scenes (see Sections 2 and 3) and derived our proposed method based on them. The validity of these assumptions, at least to some extent, can be confirmed by the fact that other ``intuitive'' despeckling methods don't work well due to information leakage (see Table~\ref{tab: quantitative analysis on real sar image}). Furthermore, based on such discussions, we have verified that our proposed method is effective not only for TerraSAR-X but also for multiple complex polarization images obtained using other sensors, which we cannot describe in detail due to confidentiality reasons.

\begin{quote}
Though the PSNR and SSIM of a so-called supervised method are recorded for simulated experimental analysis, no specific identification of the considered supervised method is provided.
\end{quote}

% われわれがSection \ref{sec:procedure}で記述している通り、擬似的なノイズを用いた実験の手順は次のように行った。
As we described in Section \ref{sec:procedure}, we conducted the experiment using pseudo noise as follows.
400 training and validation images of BSDS500~\cite{amfm_pami2011} were used for training, and 100 test images were used for evaluation. As for the synthetic speckle noise, we used noise that follows a gamma distribution with mean and variance of 1 as the equivalent of single-look speckle noise. 
We assume the image before applying the synthetic speckle noise as the ground truth. Then we can evaluate the performance of the model by comparing the GT with the image after denoising.
In this experiment, we adopt PSNR and SSIM as image quality evaluation metrics. Since optical images do not possess the concept of polarization, RGB channels were regarded as separate polarizations instead.
As there is also no complex component in optical images, the channels were replicated and considered as the real and imaginary components of each channel instead.

Specifically, the inference methods for each channel of the image differ between the two methods. In MERLIN, to replicate the assumption that all channels are independent, only two noise images independently attached to the original R channel are used for training the R channel. On the other hand, in PolMERLIN, instead of just the R channel, a total of 6 channels with independent noise attached to all RGB channels are used for training.

\begin{quote}
Moreover, the corresponding visual comparison with this supervised model is also not enlisted
\end{quote}

\begin{figure*}[htbp]
  \centering
  \tabcolsep 2pt
  \begin{tabular}{ccccc}
      \begin{minipage}[b]{0.18\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/bsds/image5/image.png}
      \end{minipage} &
      \begin{minipage}[b]{0.18\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/bsds/image5/noisy.png}
      \end{minipage} &
      \begin{minipage}[b]{0.18\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/bsds/image5/merlin.png}
      \end{minipage} &
      \begin{minipage}[b]{0.18\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/bsds/image5/ours_c.png}
      \end{minipage} &
      \begin{minipage}[b]{0.18\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/bsds/image5/ours_cs.png}
      \end{minipage} \\

      \begin{minipage}[b]{0.18\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/bsds/image3/image.png}
      \end{minipage} &
      \begin{minipage}[b]{0.18\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/bsds/image3/noisy.png}
      \end{minipage} &
      \begin{minipage}[b]{0.18\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/bsds/image3/merlin.png}
      \end{minipage} &
      \begin{minipage}[b]{0.18\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/bsds/image3/ours_c.png}
      \end{minipage} &
      \begin{minipage}[b]{0.18\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/bsds/image3/ours_cs.png}
      \end{minipage} \\

      \begin{minipage}[b]{0.18\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/bsds/image4/image.png}
        \subcaption{BSDS500}
      \end{minipage} &
      \begin{minipage}[b]{0.18\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/bsds/image4/noisy.png}
        \subcaption{Noisy}
      \end{minipage} &
      \begin{minipage}[b]{0.18\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/bsds/image4/merlin.png}
        \subcaption{MERLIN}
      \end{minipage} &
      \begin{minipage}[b]{0.18\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/bsds/image4/ours_c.png}
        \subcaption{Ours (c)}
      \end{minipage} &
      \begin{minipage}[b]{0.18\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/bsds/image4/ours_cs.png}
        \subcaption{Ours (c+s)}
      \end{minipage} \\
  \end{tabular}
  \caption{
  %BSDS500に疑似ノイズを付与してdespecklingを行ったときのRチャネルの定性的結果．MERLINによってdespecklingされた画像はRしか利用していないので少しぼけているが，提案手法はRGBチャネルの情報を利用することで画像の細部情報を比較的保ったままdespecklingに成功した．
  Qualitative results for the R channel of the BSDS500 image despeckled with pseudo-noise, showing that the image despeckled by MERLIN is blurred because only one channel is used, whereas our method uses the RGB channel and thus preserves the image detail relatively well.}
  \label{fig:detail}
\end{figure*}
As we have described in Figure \ref{fig:quality of synthetic noise}, we confirmed that the qualitative results of the proposed method, trained on the BSD500 dataset, surpass those of existing methods. Although we couldn't include them due to page limitations, we have also observed that similar results are obtained with other images as well. We show a summary of these results in Figure \ref{fig:detail}.

\begin{quote}
The paper contains self-contradicting statements on as and when required basis.
\end{quote}

We thank you for pointing that out. To avoid any misleading explanations, we have updated the relevant section to ensure consistency using mathematical expressions.

\begin{quote}
Also, the paper contains visible typing errors. One of these can be seen in the first paragraph of Section II as follows:
\end{quote}

We also thank you for pointing that out.
We have made corrections to the best of our ability regarding these issues.

\subsection{Reviewer 2}

\begin{quote}
    1. There is no mention of the resolution of the images. Kindly mention this one.
\end{quote}

We thank you for pointing this out and have added the spatial resolution to Section IV. This work uses images from the X-band SAR satellite TerraSAR-X, which has a higher spatial resolution than other C-band and L-band SAR satellites at a spatial resolution of 3m when procured in Stripmap mode. This high spatial resolution is preserved throughout the training and testing pipeline. The proposed method, similar to MERLIN, crops the images of sizes averaging $16,000 \times 16,000$ px into $256 \times 256$ px patches using a sliding window. These patches are input into the model, each resulting in an output of $256 \times 256$ px. During testing, the test images are similarly cropped to $256 \times 256$ px, but the outputs are stitched back together to create the final output size such as $16,000 \times 16,000$ px.

This means that even with a large image, despeckling can be performed without reducing its spatial resolution. We have added these descriptions to Section \ref{sec:experiments}.

\begin{quote}
2. The PSNR value is quite less compared with some existing method. It should be nearly 30dB. Clarify the reason of this low PSNR.
\end{quote}

Based on prominent papers such as "Transformer-based SAR Image Despeckling" [Perera+, IGARSS'22],
the method of image despeckling conducted in a procedure similar to our experiment achieves
a PSNR of 24.56, which is lower compared to 30dB.
However, if there are other papers that have achieved a PSNR over 30dB,
one possible reason could be the difference in the amount of noise added.

The multiple complex SAR images we handle in actual operations contain a lot of noise.
To simulate this realistic environment, we conducted performance measurements
by adding more noise than existing methods.

\begin{quote}
3. Is some pre-processing applicable to improve the PSNR? ( i.e. Application of conventional filters before applying user’s own noise reduction process)
\end{quote}

Our method adopts a self-supervised learning approach for despeckling under the assumption of statistical independence across channels and within the image space. While it is possible to apply classical whitening filters, like the median filter, prior to implementing our proposed method, there's a risk that such filters might inadvertently remove valuable information beyond just the noise. Additionally, what these filters inherently assume is the spatial independence wherein the noise of the current pixel is added independently of the noise in the surrounding pixels. This assumption aligns with that of our method. Therefore, it can be inferred that our method potentially learns such classical filtering behaviors within the internal representations of the trained Deep Neural Network (DNN).

\begin{quote}
4. Following papers are related with the noise reduction from the remote sensing images and
provides excellent result in terms of PSNR. Authors may study these papers and include in the
manuscript.
\end{quote}

We thank you for pointing this out. Although the amount of noise added differs, and thus cannot be compared in general, there is no doubt that this is a relevant study. We have cited those studies in our main paper.

==> sec/related_work.tex <==
\section{Related Work}
\label{sec:related_work}

\subsection{Self-Supervised Image Denoising}
Since it is hard to obtain noise-free images from noisy sensors for supervised learning, many self-supervised image denoising methods have been proposed in recent years.
Noise2Noise~\cite{pmlr-v80-lehtinen18a} trains a denoising model using multiple noisy images that capture the same scene. 
\cite{laine2019high} proposes to utilize partial information about the blind spot pixel.
Noise2Void~\cite{krull2019noise2void}, Speckle2Void~\cite{molini2021speckle2void}, and Noise2Self~\cite{pmlr-v97-batson19a} make the model trainable from a single noisy image. These methods train the model by predicting a ``blind-spot'' pixel that is masked out from the NN input. 
We improve the performance by partially incorporating the ideas from these studies that intersect with the core of our method.

Approaches that do not use blind spots have also been actively studied. \cite{Moran_2020_CVPR,Xu2020NoisyasCleanLS} added additional noise to the original noise image to generate noisy-noisy pairs. Neighbor2Neighbor~\cite{Huang_2021_CVPR} used subsampling to generate noisy-noisy pairs, and CVF-SID~\cite{Neshatavar_2022_CVPR} split the noise image into noise-free, signal-dependent, and signal-independent noise. Unlike these approaches, our method performs accurate despeckling by hiding multiple channels and training a model to recover them.

\subsection{SAR Image Despeckling}
Over the years, various image denoising techniques have been proposed to address speckle noise in SAR images. 
Traditional approaches to despeckling involved filter-based methods~\cite{LEE198124,4767223,1165131}, which were later superseded by wavelet-based methods~\cite{1105905, 413278} that achieved superior performance.

Many deep learning methods have been proposed in the area of despeckling.
SAR-CNN~\cite{8128234} is a supervised learning method that applies CNN to despeckling.
Starting from SAR-CNN, various supervised despeckling methods~\cite{wang2017sar,perera2022transformer,perera2022sar} have been proposed.
Supervised learning targets a clean (noise-free) SAR image, but since a clean SAR image does not exist, it is necessary to prepare a virtual clean SAR image by averaging multi-temporal SAR images.
Due to the difficulty of obtaining multi-temporal images, self-supervised despeckling, which can be trained using only noisy SAR images, has been actively studied.
Speckle2Void~\cite{molini2021speckle2void} proposes a framework that can learn directly from noisy SAR images by assuming a speckle noise model like ~\cite{581981} and using a blind-spot network.
MERLIN\cite{dalsasso2021if} and SAR2SAR~\cite{dalsasso2021sar2sar} are extensions of Noise2Noise to despeckling.
SAR2SAR is a method for generating noisy-noisy pairs from multi-temporal SAR images.
MERLIN is a method for learning noisy-noisy pairs from single-polarization complex SAR images using Noise2Noise~\cite{pmlr-v80-lehtinen18a}, because the real and imaginary components of a single-polarization complex SAR image are independent.
\cite{meraoumia2022multi} extends MERLIN to multi-temporal SAR images.
These Noise2Noise-inspired methods are powerful, but require independent noise image pairs.
SAR-IDDP~\cite{9911647} proposed a high quality method using DIP~\cite{Ulyanov_2018_CVPR} that does not require noisy-noisy pairs.
The above despeckling methods are based on single-polarization SAR images, where modeling of the joint distribution is simple.
